Latexify Math: Mathematical Formula Markup Revision to Assist Collaborative Editing in Math Q&A Sites

Collaborative editing questions and answers plays an important role in quality control of Mathematics Stack Exchange which is a math Q&A Site. Our study of post edits in Mathematics Stack Exchange shows that there is a large number of math-related edits about latexifying formulas, revising LaTeX and converting the blurred math formula screenshots to LaTeX sequence. Despite its importance, manually editing one math-related post especially those with complex mathematical formulas is time-consuming and error-prone even for experienced users. To assist post owners and editors to do this editing, we have developed an edit-assistance tool, MathLatexEdit for formula latexification, LaTeX revision and screenshot transcription. We formulate this formula editing task as a translation problem, in which an original post is translated to a revised post. MathLatexEdit implements a deep learning based approach including two encoder-decoder models for textual and visual LaTeX edit recommendation with math-specific inference. The two models are trained on large-scale historical original-edited post pairs and synthesized screenshot-formula pairs. Our evaluation of MathLatexEdit not only demonstrates the accuracy of our model, but also the usefulness of MathLatexEdit in editing real-world posts which are accepted in Mathematics Stack Exchange.

==> motivation.tex <==
\section{Motivation}
\label{motivation}


\site is one of the most popular Q\&A sites for mathematics.
Millions of mathematicians share and learn mathematics knowledge in this discussion site\footnote{\url{https://math.stackexchange.com/}}. 
An important reason of using \site is that the posts are well maintained by the community in the site. 
Once a question or answer is posted, not only the post owner can edit the content, other post editors can also collaboratively maintain the post content.
According to our empirical study in Section~\ref{sec:empiricalStudy}, nearly half \hk{of the} posts have been edited more than once.
By analyzing the frequent words and topics from the editing comments, we find that many edits are domain-specific i.e., highly related to the math formula.
\textcolor{blue}{Among all these edits, three editing patterns are very common i.e.,  latexifing formulas, revising LaTeX and transcribing screenshots into a mathematical typesetting textual format e.g. using Mathjax~\cite{CervoneDavide2012MAPf} for rendering the Latex, }
% Among all these edits, one editing pattern is very common i.e., transcribing the mathematics formula into a mathematical typesetting textual format e.g. using Mathjax~\cite{CervoneDavide2012MAPf} for rendering the Latex.
\begin{figure}
\centering
\subfigure[plain text] { \label{cpr:a}
\includegraphics[width=0.25\columnwidth]{figs/natural_math.png}
}
\subfigure[screenshot] { \label{cpr:b}
\includegraphics[width=0.25\columnwidth]{figs/blurred_image.pdf}
}
\subfigure[Mathjax] { \label{cpr:c}
\includegraphics[width=0.25\columnwidth]{figs/clear.pdf}
}
\caption{ 
Comparison of plain text, screenshot and Mathjax} 
% \chen{need another example about plain text describing the math formula}}
\label{fig:compare}
\end{figure}

\textcolor{blue}{Translating natural language can highly improve the readability of posts.
Compared with natural language, as shown in Fig ~\ref{fig:compare}, LaTeX can render better visualization effect, which helps users easily read the math formulas.}
\textcolor{blue}{Correcting the errors in LaTeX formulas help improve the quality of post contents. 
Tiny token errors may result in the wrong rendering of LaTex formulas, which cannot be understood by the readers.
Sometimes, with errors, the rendering of LaTeX formulas may show totally different meaning, which leads reader misunderstand the content of posts.}

Converting a posted mathematics formula screenshot to Latex brings many benefits to the site.
First, as shown in Fig~\ref{fig:compare}, transcribing the mathematics formula screenshot makes the site easier to read for everyone, as users can zoom in or out for a clearer view without blurring the formula.
Such readability can help other users better understand the question, resulting in higher possibility of responses.
Second, this machine-readability also makes the text easier to register and index by search-engine crawlers. 
This in turn makes the post easier to search for and easier to be found by other users, and this, therefore, makes the post more useful for a broader cross-section of internet users.
% Third, such a screenshot transcribing feature would make the questions more accessible to users with vision impairment, where the formula can be spoken by screen reader.
% The users with visual impairments, ranging from difficulty reading all the way to complete blindness, need to be able to use the internet and study maths~\cite{AlajarmehNancy2012Dmma}.
% When visiting the website, they mainly rely on assistive technology such as screen readers which can only read the text, rather than the image.
% Using proper typesetting (including good use of Markdown and Mathjax) provides additional HTML syntax that those assistive technologies can use to give a more meaningful account of the content on the page.



The writing guide in \site  provides a tutorial~\cite{tutorial} for using Mathjax to format the mathematics formulas.
However, considering the diversity of characters and formats involved in LaTeX formatting and the learning curve, it requires significant manual effort to transcribe screenshots, especially for the novice users.
% Even for experienced users, it is difficult for them to convert a screenshot with a complicated mathematics formula to Latex and that process may be error prone.
\textcolor{blue}{Even for experienced users, it is difficult for them to correct the errors in LaTeX formulas, translate natural language to LaTeX formulas and convert a screenshot with a complicated mathematics formula to Latex and that process may be error prone.}

% Therefore, an automatic approach is needed to assist the image transcribing.
\textcolor{blue}{Therefore, an automatic approach is needed to help keep formal LaTeX format.}
It will help post owners and post editors to improve their editing efficiency.
Furthermore, such an image transcribing tool is also a great way to lower the engagement bar for novice users to the \site Q\&A site.%\hk{this sentence is not very clear to me}

%\hk{1) the following paragraph makes the intro very long, 2) the next paragraph which talks bout the findings of this work based on the empirical studies is better connected to the previous paragraph. It seems too detailed for here I think. Can this paragraph be discussed in the methodology section later?} \chen{Need to tell more about the empirical study.}





==> practice.tex <==
\section{Assist Post Editors with Image Conversion}
\hk{I would add this as a subsection in section 6, as a real world evaluation, or rename this to reflect its based on a real usecase}
Having established the confidence in the quality of rendered LaTeX formulas by our tool, we would like to further investigate whether the recommended edits by our tool can assist post editors to successfully convert formula images to LaTeX characters in practice.

To that end, we conducted a small-scale field study, in which the first author who have no experience in \site, acts as a post editor. 
We randomly selected 40 posts which contain formula images which has not been converted to LaTeX. 
%These posts are of reasonable size, and the human effort to manually collect these posts and submit the post edits is manageable. 
In \site, each question can have up to 5 tags to describe its topic. 
The 40 selected posts contain 135 tags in total (if the post is the answer, we take tags from its corresponding question) and 92 of these tags are unique.
This indicates that the 40 selected posts cover a diverse set of mathematical topics. 
In fact, these posts contain many mathematical terms that are beyond the expertise of the first author.
For these 40 posts, there are 42 formulas images in total.
Only two posts have two unconverted formula images, other posts have one formula image.

In Mathematics Stack Exchange, novice post editors have to submit their post edits for peer review. 
According to the \site policy~\cite{math}, to guarantee the quality of post edits, a post edit will be accepted only if at least two trusted contributors approve the edit otherwise it will be rejected. 
The first author uses our model to generate screenshot conversions for the selected 40 posts, based on which he edits the posts and submit the post edits to the community for approval.
Our field study lasts for three days as each user in \site can submit at most 5 post edits at the same time. 
%We cannot submit more post edits until some submitted post edits are accepted or rejected.


% To test the ability of our model in help users edit the post content, we conduct another real-world experiment. Firstly, we search the posts in Math Stack Exchange, and collect formula screenshots that have not been converted to LaTeX formulas. Secondly, we convert the collected formula screenshots to LaTeX characters using our model. Thirdly, we edit the original post and replace the original formula images with converted LaTeX formulas, and we see if the revision will be accept or not. To test the ability of our model in helping collaborative editing, we search posts that contains unconverted formula image in Math Stack Exchange site. 

% \subsection{Result}
\begin{figure}%[ht]
	\centering
	\includegraphics[scale=0.2]{figs/error2.pdf}
	%\vspace{-3mm}
	\caption{Example of rejected revision}
	%\vspace{-3mm}
	\label{fig:err2}
\end{figure}


Among the 40 submitted post edits, 38 (95\%) were accepted and 2 (5\%) were rejected. 
Records of some edits are shown in Fig \ref{fig:web}.
For the two rejected edits, the original images have special notation in the formulas.
Although our tool recommend the correct LaTeX formulas, the notations in the formulas images are missed.
Figure \ref{fig:err2} shows one example with yellow notation of some parts of the formula for illustrating some concept.
Since our revised LaTeX formula miss the annotation which is important for this post, the revision is not accepted.
But for the 38 accepted post edits, the trusted contributors believed that they contain sufficient edits that significantly improve the post quality, and thus approved them.
The acceptance of our proposed edits demonstrate the usefulness of our tool in transcribing the formula screenshots.


% We searched 40 posts, and edits these posts by replacing the original formula images with LaTeX characters generated by our model. After we submitted these edits, 28 edits are accepted, and 12 edits are rejected. The accepted percentage is 70\%. Figure \ref{fig:web} is an example of accepted editing.
% \chen{Why are there so many edits rejected? Please summarize the reasons!}

\begin{figure}%[ht]
	\centering
	\includegraphics[scale=0.3]{figs/webpost2.pdf}
	%\vspace{-3mm}
	\caption{Example of Assisting Post Editors with Image Conversion}
	%\vspace{-3mm}
	\label{fig:web}
\end{figure}
